Grounding Partially-Defined Events in Multimodal Data

How are we able to learn about complex current events just from short snippets of video? While natural language enables straightforward ways to represent under-specified, partially observable events, visual data does not facilitate analogous methods and, consequently, introduces unique challenges in event understanding. With the growing prevalence of vision-capable AI agents, these systems must be able to model events from collections of unstructured video data. To tackle robust event modeling in multimodal settings, we introduce a multimodal formulation for partially-defined events and cast the extraction of these events as a three-stage span retrieval task. We propose a corresponding benchmark for this task, MultiVENT-G, that consists of 14.5 hours of densely annotated current event videos and 1,168 text documents, containing 22.8K labeled event-centric entities. We propose a collection of LLM-driven approaches to the task of multimodal event analysis, and evaluate them on MultiVENT-G. Results illustrate the challenges that abstract event understanding poses and demonstrates promise in event-centric video-language systems.

==> content/99_method_notes_temp.tex <==
\section{Role Localization Approaches}
\label{temp_sec:method}


\alex{Put intro sentence / transitory sentence here}. We introduce a suite of finetuned video language models based on TimeChat \cite{ren2024timechat} encoding architecture. Due to the similar nature of temporal span retrieval and video grounding, we finetune TimeChat on temporal video grounding data from 4 datasets \cite{}\alex{\todo{cite charades and the other ones}} (\autoref{tab:???} as TimeChat$_{\text{tvg}}$. We then further finetune this model specialized for temporal video grounding on additional silver data: ActivityNet Templates \autoref{appendix:activitynet} (\autoref{tab:???} as TimeChat$_{IE}$. 

While video language models are generalists and can produce strong text output, they still lag behind video-based decoders. To baseline these video-centric models, we baseline two state-of-the-art models with strong abilities to generalize to new domains VDI \cite{luo2023generalisable} and MMN \cite{wang2021negative}. 


\section{eval metrics}
\paragraph{Template filling evaluation metric.} We define an IoU-based F1 score for role localization as a template filling task. We denote the Agreement, $\alpha$, as the $\frac{Intersection}{Union}$. We define the set of gold role fillers $G = \{R_1, R_2, \ldots, R_N\}$, where $R_i={r_i^1, r_i^2, \ldots, r_i^m}$ is the set of gold role fillers for the $i$th role in the template. 

\alex{before the F1 score, we should probably do some matching within a predicted role set to determine the highest agreement score.}



\begin{equation}
    TP = \sum_{R_i \in G; R_i \ne \emptyset \cap P_i \ne \emptyset}\alpha 
\end{equation}

\alex{We do $\frac{1-\alpha}{2}$ in order to not count the disagreement twice}
\begin{equation}
    FP = \sum \frac{1-\alpha}{2} + \sum 1
\end{equation}

\begin{equation}
    FN = \sum \frac{1-\alpha}{2} + \sum 1
\end{equation}


==> content/old_experiments.tex <==
\section{Experiments}
\label{sec:experiments}
\subsection{Text Span Retrieval}
\label{sub-sec:exps:text}

We evaluate the methods detailed in Section 5.1 on the task of text evidence retrieval, and report results in Table \ref{tab:text-exps}. We find that most of the LLMs perform relatively well on the task, and do not benefit substantially from few-shot prompting. For some of the models, few-shot prompting hurt performance. High recall typically indicates longer retrieved spans, potentially full sentences, whereas precision indicates that single-word spans were likely more frequent. Of the three task stages, text span extraction appears to be the easiest, which is unsurprising given the recent strides made in high-level inference over noisy text data.


\subsection{Temporal Retrieval}
\label{sub-sec:exps:temporal}
We then evaluate the Section 5.2 methods on the task of temporal retrieval using the \dsetname dataset. We report results in \autoref{tab:temporal}. We find that VideoLLMs are capable of generalizing to the temporal retrieval task when it matches the task of temporal video grounding observed during instruction tuning. We see the best model in performance when the VideoLLM undergoes additional instruction tuning for the Charades \cite{zhang2019temporal}. However, when the VideoLLM is tuned further on additional temporal video grounding data, it loses its ability to generalize to \dsetname. This is due to the out-of-distribution nature of \dsetname. Traditional temporal video grounding focuses on entity-specific tasks, but the \dsetname{} ontology covers a broader event spectrum, some of which are not human-centric. We offer a further breakdown of the performance of the temporal retrieval task across the languages and template types in \autoref{sub-appendix:additional-results:temporal}. 



\subsection{Spatial Retrieval}
\label{sub-sec:exps:spatial}

Finally, we evaluate the methods in Section 5.3 on the task of spatial retrieval with results in Table X. We evaluate on 12,400 frames in total.

<Discussion>

\subsection {Discussion}
\label{sub-sec:exps:discussion}

==> prompts/p01_acnet_templates.tex <==
\begin{figure*}
\noindent\fbox{%
    \parbox{\textwidth}{%
\textbf{ActivityNet Templates generation}\\

\footnotesize
{\tt
The following text passage mentions the activity of "<activity>".\\

TEXT PASSAGE:
"<summary>"\\

Please write the nouns mentioned in the text, as they are written, that could be answers to the following questions. If none of the nouns work as answers, write N/A. Write your answers in list format, e.g.,
1. <Noun 1>, <Noun 2>
2. N/A
3. <Noun 3>
...\\

QUESTIONS:
<questions>\\

ANSWERS:
}
}}

\caption{}
\label{prompt:acnet_templates}
\end{figure*}

==> prompts/p03_temporal_span_labeling.tex <==
\begin{figure*}
\noindent\fbox{%
    \parbox{\textwidth}{%
\textbf{Temporal span labeling}\\

\footnotesize
{\tt
...
}
}}

\caption{}
\label{prompt:temporal-spans}
\end{figure*}

==> prompts/p05_obj_mapping.tex <==
\begin{figure*}
\noindent\fbox{%
    \parbox{\textwidth}{%
\textbf{Spatial entity role mapping}\\

\footnotesize
{\tt
The following objects are present in an image of a <activity>.\\

OBJECTS:
"<summary>"\\

Please write the objects in the list, as they are written, that could be answers to the following questions. If none of the nouns work as answers, write N/A. Write your answers in list format, e.g.,
1. <Noun 1>, <Noun 2>
2. N/A
3. <Noun 3>
...\\

QUESTIONS:
<questions>\\

ANSWERS:
}
}}

\caption{}
\label{prompt:mapping}
\end{figure*}
